BiPACE: Bisimulation-Guided Policy Optimization with Action Counterfactual Estimation for LLM Agents

Stepwise group-based RL is an attractive way to train long-horizon LLM agents without a learned critic: it reuses multiple sampled rollouts to estimate local advantages. Its weakness is less visible but more fundamental: every group-relative estimator assumes that the steps it compares are equivalent for credit assignment. We show that current agentic variants violate this assumption through a state-action credit mismatch. The observation-hash partition is overly fine on the state side, creating singleton groups with zero step-level signal, while a single within-group mean is too coarse on the action side, mixing state-value estimation with action-specific credit. We introduce BiPACE (Bisimulation-Guided Policy Optimization with Action Counterfactual Estimation), a drop-in advantage estimator that fixes both sides without adding a critic, auxiliary loss, or extra rollouts. BiGPO clusters steps by cosine distance in the actor's own hidden-state geometry, an empirical policy-induced proxy for bisimulation that substantially lowers the singleton rate left by observation hashing. PACE then recenters returns within each behavioral cluster using action-conditioned peer baselines; its Q-style instance estimates a local Q(s,a)-V(s) nonparametrically. On ALFWorld/Qwen2.5-7B, BiPACE_Q raises overall validation success from GiGPO's 90.8 to $97.1\pm0.9$ over three seeds, and crosses the 95% threshold on every seed, which GiGPO never does within the same budget. On Qwen2.5-1.5B it reaches $93.5\pm1.2$ versus GiGPO's 86.7, and on WebShop and TextCraft it improves over GRPO and GiGPO at both model scales. The measured BiPACE-specific overhead is 11.3% of a single training-step wall time. Yet it changes the estimator's comparison unit from surface identity to approximate behavioral equivalence plus action-side counterfactuals. The code is available at https://github.com/TianxiangZhao/BiPACE.

==> Arxiv/preamble_defs.tex <==
% Shared paper macros and style tokens. Keep this file loaded from the
% preamble, after xcolor/colortbl and before hyperref/title use.

\makeatletter
\@ifundefinedcolor{linkblue}{\definecolor{linkblue}{RGB}{34,79,135}}{}
\@ifundefinedcolor{codegray}{\definecolor{codegray}{RGB}{244,245,247}}{}
\@ifundefinedcolor{tblhead}{\definecolor{tblhead}{RGB}{240,243,247}}{}
\@ifundefinedcolor{tblgroup}{\definecolor{tblgroup}{RGB}{247,248,250}}{}
\@ifundefinedcolor{tblours}{\definecolor{tblours}{RGB}{236,244,255}}{}
\@ifundefinedcolor{tblref}{\definecolor{tblref}{RGB}{248,248,248}}{}
\makeatother

\providecommand{\R}{\mathbb{R}}
\providecommand{\E}{\mathbb{E}}
\providecommand{\Var}{\mathrm{Var}}
\providecommand{\KL}{\mathrm{KL}}
\providecommand{\dpi}{d_\pi}
\providecommand{\bigpo}{\textnormal{\scshape BiGPO}}
\providecommand{\bipace}{\textnormal{\scshape BiPACE}}
\providecommand{\gigpo}{\textnormal{\scshape GiGPO}}
\providecommand{\hgpo}{\textnormal{\scshape HGPO}}
\providecommand{\hcapo}{\textnormal{\scshape HCAPO}}
\providecommand{\istar}{\textnormal{\scshape iStar}}
\providecommand{\mico}{\textnormal{\scshape MICo}}

\providecommand{\code}[1]{\colorbox{codegray}{\texttt{\small #1}}}

% Compact-but-breathing booktabs default; opt in per table.
\providecommand{\tabstretch}{\renewcommand{\arraystretch}{1.15}}
\providecommand{\tblgroup}[2]{\rowcolor{tblgroup}\multicolumn{#1}{@{}l}{\emph{#2}}}
\providecommand{\missing}{\textcolor{black!40}{\textemdash}}

% Footnote marks for partial-completion runs.
\providecommand{\seedone}{\textsuperscript{\dag}}
\providecommand{\seedtwo}{\textsuperscript{\ddag}}


==> Arxiv/sections/01_intro.tex <==
% !TEX root = ../main.tex
% =====================================================================
\section{Introduction}\label{sec:intro}

Reinforcement learning (RL) post-training of large language models has
recently moved beyond single-turn reasoning into the harder
\emph{agentic} regime: long-horizon, partially observed, multi-turn
interaction with tools, web pages, simulated households, and games.
The central obstacle is assigning a sparse terminal reward to the
intermediate decisions that made the trajectory succeed or fail.
Group-based RL
methods such as RLOO-style leave-one-out
estimators~\citep{kool2019buy,ahmadian2024back} and
GRPO~\citep{shao2024deepseekmath} are appealing because they avoid a
learned value network. Recent agentic variants such as
\gigpo{}~\citep{feng2026group} and \hgpo{}~\citep{he2026hierarchy} push
this idea to the step level by comparing rollout steps inside groups.
Their performance, however, depends on a choice that is often treated
as an implementation detail: which steps are grouped together for that
comparison.

These estimators share an implicit assumption: if two step records are
placed in the same group, then they are interchangeable for credit
assignment. In long-horizon agent environments, this assumption fails
in two coupled ways. \textbf{State side:} observation identity is a
convenient but overly sparse proxy for value equivalence. Group
baselines are reliable when grouped states share continuation value, a
condition formalized by \emph{bisimulation}
\citep{givan2003equivalence,ferns2004metrics}; observation keys impose
a strictly finer equivalence than bisimulation requires, splitting many
reusable states into isolated singletons. \textbf{Action side:} even
when states are comparable, the usual within-group mean assigns the
same baseline to all actions, ignoring that different actions from the
same state can induce different futures. We call this two-sided
failure the \emph{state-action credit mismatch}.

This mismatch is detectable as a diagnostic metric during training,
independently of the final task reward. In our \gigpo{} reproduction
diagnostics on \textsc{ALFWorld}, $34.2\%$ of clusters are singletons
at iteration 10, and the fraction remains $20.7\%$ at iteration 140.
Since singleton clusters produce zero step-level advantage, exact
observation hashes discard local signal when the policy needs it most.
On \textsc{TextCraft}, where observations are sparser, exact hashes
isolate even more records and expose fewer matched pairs (detailed
in \cref{sec:mechanism}).

We propose \bipace{} (\emph{Bisimulation-Guided Policy Optimization
with Action Counterfactual Estimation}), a drop-in advantage estimator
that treats step-level credit as two local problems: state aggregation
and action recentering. \textbf{On the state side}, \bigpo{} replaces
observation hashing with cosine clustering on the actor's own hidden
state $\phi_\theta(s_t)$, taken at a late intermediate layer selected
once per backbone (\cref{app:hparams,app:scale-calibration}), which
serves as an empirical proxy for the behavioral metrics studied by
\citet{castro2021mico}. \textbf{On the
action side}, PACE partitions each behavioral cluster by the executed
action and replaces the cluster mean with a nonparametric
counterfactual baseline. The two halves are coupled: PACE needs
behaviorally comparable state peers, and state aggregation is most
useful when the residual variation inside a state neighborhood is
action-specific rather than noise.
Our main contributions are summarized as follows:
\begin{itemize}
\item \textbf{\emph{Identifying state-action credit mismatch.}}
  We show that stepwise group-based RL conflates state aggregation with
  action recentering, and that exact observation hashing is the wrong
  state equivalence relation, splitting reusable states into singletons
  that carry no step-level signal.
\item \textbf{\emph{Proposing a drop-in advantage estimator.}}
  We introduce \bipace{}, which makes two local replacements:
  \bigpo{} clusters actor-hidden fingerprints as a policy-induced
  bisimulation proxy, and PACE adds an action-conditioned peer baseline
  inside each cluster.
\item \textbf{\emph{Analyzing the estimator.}}
  We bound the state-side bias by $O(\varepsilon)$ under a
  \mico{}-Lipschitz assumption, recover \gigpo{} as the
  $\varepsilon{=}0$ limit, quantify the singleton signal loss, and show
  Q-style PACE is exact under exact bisimulation.
\item \textbf{\emph{Achieving strong empirical performance.}}
  \bipace$_{\text{Q}}$ gains $+6.3$pp on \textsc{ALFWorld}/Qwen2.5-7B
  ($97.1{\pm}0.9$ vs.\ $90.8$) and $+6.8$pp on 1.5B, and improves over
  GRPO and \gigpo{} on \textsc{WebShop} and \textsc{TextCraft} at both
  scales, at only $11.3\%$ step overhead.
\end{itemize}


==> Arxiv/sections/02_related.tex <==
% !TEX root = ../main.tex
% =====================================================================
\section{Related Work}\label{sec:related}

{\sloppy
\paragraph{Group-relative RL for LLM agents.}
\bipace{} builds on critic-free group-relative RL, including
GRPO~\citep{shao2024deepseekmath}, \gigpo{}~\citep{feng2026group}, and
\hgpo{}~\citep{he2026hierarchy}. These methods compare sampled
returns inside groups but keep the state equivalence relation discrete;
\bipace{} replaces that relation with a policy-induced behavioral
partition. The state side follows the value-preserving bisimulation
view~\citep{ferns2004metrics,castro2021mico,zhang2020learning}, while
PACE gives a nonparametric analogue of action-conditioned
counterfactual baselines studied in COMA/CCPO and related work~\citep{foerster2018counterfactual,li2026counterfactual}. Other
agent-credit methods alter the learning signal or optimizer~\citep{tan2026hindsight,liu2025agentic,wei2025reinforcing,yu2026dapo};
\bipace{} instead changes which step records are compared. Extended
discussion appears in \cref{app:extended-related}.
\par}


==> Arxiv/sections/03_preliminaries.tex <==
% !TEX root = ../main.tex
% =====================================================================
\section{Background Details}\label{app:preliminaries}

\subsection{Multi-turn LLM agent decision process}
We consider an episodic POMDP $\mathcal{M} = (\mathcal{S},
\mathcal{A}, P, r, \gamma, T)$ in which an LLM policy
$\pi_\theta(a_t \mid s_t)$ produces a textual action $a_t$ given an
observation $s_t$, and the environment returns a next observation
$s_{t+1}$, a (typically sparse) reward $r_t$, and a done flag.
Throughout, $s_t$ denotes the agent-visible observation, which plays
the role of state for estimation purposes. We follow
\citet{feng2026group} in a \emph{step-independent} input formulation:
each step's prompt is constructed from the current observation and a
(possibly summarized) history, enabling horizons of $50{+}$ steps.

For each prompt $p$ we sample $G$ trajectories
$\tau^{(1)}, \ldots, \tau^{(G)}$ of (possibly varying) lengths
$T^{(g)}$. In the terminal-only reward setting we focus on, the
trajectory return is $R(\tau) = r_{T-1}$
(e.g., $1$ on success and $0$ otherwise on \textsc{ALFWorld}).

\paragraph{GRPO and \gigpo{}.}
The GRPO episode-level advantage and the \gigpo{} step-level advantage
are defined in the main paper (Eqs.~1--2 and the surrounding
discussion in \S\,\ref{sec:method}). The two failure modes of
exact observation hashing that motivate \bigpo{}---singleton clusters
and paraphrase splitting---are analyzed in \S\,\ref{sec:method-mismatch}.

\subsection{Bisimulation and the \mico{} metric}
\label{app:prelim-bisim}
A binary relation $E$ on states is a \emph{bisimulation} if $sEs'$
implies $r(s,a)=r(s',a)$ and
$\sum_{s_+\in[s_+]_E} P(s_+\mid s,a) =
\sum_{s_+\in[s_+]_E} P(s_+\mid s',a)$
for all $a$~\citep{givan2003equivalence}. Aggregating bisimilar states
preserves $V^\pi$ (and indeed $Q^\pi$ for every policy); bisimulation
is thus a sufficient---if conservative---equivalence for
value-preserving state aggregation.

\citet{castro2021mico} introduce the \emph{\mico{} distance} $\dpi$, a
tractable sample-based approximation satisfying the value-difference
bound
\begin{equation}
\bigl| V^\pi(s) - V^\pi(s') \bigr| \;\le\; \dpi(s, s').
\label{eq:app-mico-bound}
\end{equation}
\bigpo{} uses an empirical proxy for $\dpi$ derived from the policy's
own hidden representation; \cref{prop:bigpo-bias-var} formalizes the
resulting bias bound on the step-level advantage estimator.


==> Arxiv/sections/04_method.tex <==
% !TEX root = ../main.tex
% =====================================================================
\section{Method: \bipace{}}\label{sec:method}

This section first isolates the estimation issue that \bipace{}
targets, then describes the two local replacements that constitute
the method.

\subsection{Estimator setup}
\label{sec:method-setup}
For each prompt group $p$, GRPO samples trajectories
$\{\tau^{(g)}\}_{g=1}^G$ and standardizes terminal returns within the
group,
\begin{equation}
A^{\mathrm{ep}}(\tau^{(g)}) =
\frac{R(\tau^{(g)})-\mu_p}{\sigma_p+\delta},
\quad \mu_p,\sigma_p \text{ over } \{R(\tau^{(g)})\}_{g=1}^G .
\label{eq:episode-adv}
\end{equation}
\gigpo{} adds a step-level term by collecting all step records in the
same prompt group and partitioning them by exact observation hash:
$\mathcal{C}_p = \big\{\,\{i:\mathrm{hash}(s^{(i)})=h\}: h\in \mathrm{Hash}(\{s^{(i)}\}_{i\in p})\,\big\}$.
For each cluster $C\in\mathcal{C}_p$, it normalizes the return-to-go
$R_t^{(i)}$ locally:
\begin{equation}
A^{\mathrm{step}}(i) =
\frac{R_t^{(i)}-\mu_C}{\sigma_C+\delta}, \quad i\in C .
\label{eq:step-adv}
\end{equation}
All changes below keep this GRPO/GiGPO training loop intact and
replace only the partition and the local baseline used by
\cref{eq:step-adv}. Extra background on the agent decision process,
GRPO, and bisimulation appears in \cref{app:preliminaries}.

\subsection{The state-action credit mismatch}
\label{sec:method-mismatch}
\gigpo{} improves over trajectory-level GRPO by computing a
step-level advantage within groups of rollout steps that share the
same current observation. This design assumes that two step records in
the same group are exchangeable for credit assignment. In agentic
tasks, the assumption breaks in two complementary ways.

\textbf{State side.}
Exact observation identity is a strict and sparse proxy for value
equivalence. If two observations differ only in surface form, they are
placed in different groups even when they induce the same continuation
value. Conversely, when the exact-key partition produces singleton
groups, the within-group baseline in \cref{eq:step-adv} degenerates to
zero and the step contributes no step-level gradient. Thus the state
partition controls both bias and usable signal.

\textbf{Action side.}
Even when a group contains behaviorally comparable states, the usual
within-group mean assigns the same baseline to all actions. This is
too coarse: two actions from the same state neighborhood can lead to
different futures, and recentering both against one group mean mixes
state-value estimation with action-specific credit. The desired
quantity is closer to a local counterfactual advantage,
$Q(s,a)-V(s)$, rather than a raw deviation from the cluster average.

\bipace{} addresses these two sides jointly. On the state side,
\bigpo{} replaces the observation-hash partition with a
policy-induced behavioral partition. On the action side, PACE replaces
the within-cluster mean with an action-conditioned counterfactual
baseline.

\subsection{BiPACE overview}
\label{sec:method-overview}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/method_overview.pdf}
\captionsetup{font=footnotesize}
\caption{\textbf{Method overview.}
\bipace{} makes two local replacements to the GiGPO step-level
estimator. \textbf{Left:} A prompt group provides step records
($s_t^{(i)}, a_t^{(i)}, R_t^{(i)}$) across $G$ rollouts; chip colors
encode bisimulation class. \textbf{Middle:} \bigpo{} extracts the
actor's normalized hidden state $\phi_\theta(s)$ at a fixed late layer
and clusters by cosine distance, forming behavioral state neighborhoods
$\mathcal{C}_1,\mathcal{C}_2,\ldots$ \textbf{Right:}
PACE recenters returns inside each cluster by the executed action key;
the Q-style form estimates $\widehat Q(s,a)-\widehat V(s)$.
Only the step-level advantage changes; the PPO objective is unchanged.}
\label{fig:method-overview}
\end{figure*}

\begin{tcolorbox}[
  colback=tblours!55,
  colframe=linkblue!38,
  boxrule=0.55pt,
  arc=1mm,
  left=7pt,
  right=7pt,
  top=6pt,
  bottom=6pt]
\textbf{\bipace{} in one line.}
For each prompt group, \bipace{} first clusters step records by the
actor's own hidden-state geometry (\bigpo{}), then computes the
step-level baseline inside each cluster conditional on the executed
action (PACE). Everything outside the advantage estimator is identical
to \gigpo{}.
\end{tcolorbox}

\Cref{fig:method-overview} traces the full pipeline.
\textbf{Left.}
$G$ rollouts from a shared prompt $p$ yield step records
$(s_t^{(i)}, a_t^{(i)}, R_t^{(i)})$; chip colors encode bisimulation
class.
\textbf{Middle (\bigpo{}).}
The actor's hidden state $f_\theta(s_t)$, taken at a fixed late layer
and $\ell_2$-normalized to $\phi_\theta(s)$, is greedily clustered by
cosine distance: records sharing behavioral geometry merge into
$\mathcal{C}_1$; outliers seed a new cluster~$\mathcal{C}_2$.
\textbf{Right (PACE).}
Inside $\mathcal{C}_1$, records split by action key $\kappa(a_i)$:
same-action peers $C^{=}(i)$ estimate $\widehat Q(s,a_i)$, the full
cluster estimates $\widehat V(s)$, and the counterfactual step
advantage $\hat A_i^S = \widehat Q(s,a_i)-\widehat V(s)$ enters the
additive combination $A_i^{\bipace{}} = A_i^{\mathrm{ep}} +
w\cdot\hat A_i^S$ with an \emph{unchanged} PPO objective.

\subsection{State-side grouping with \bigpo{}}
\label{sec:method-bigpo}
\bigpo{} replaces exact observation hashing with a behavioral
fingerprint extracted from the policy itself. Let
$f_\theta : \mathcal{S}\to\R^D$ be the function that maps the current
prompt $s_t$ to the actor LLM's hidden state at the final prompt
token, taken at a fixed late intermediate layer chosen once per
backbone (layer $-8$ for Qwen2.5-7B, $-12$ for Qwen2.5-1.5B;
calibration details in \cref{app:hparams,app:scale-calibration}). We use the normalized representation
$\phi_\theta(s) = f_\theta(s)/\|f_\theta(s)\|_2$.
This representation moves with the policy being optimized and is
available as a by-product of the actor forward pass, requiring no
learned critic or auxiliary model.

For each prompt group $p$, \bigpo{} computes the partition
\begin{equation}
\mathcal{C}_p^{\bigpo} \;=\; \mathrm{Cluster}_\varepsilon\big(
\{ \phi_\theta(s^{(i)}) : i \in p \}, \; d_{\cos}\big),
\label{eq:bigpo-clusters}
\end{equation}
where $d_{\cos}(u,v)=1-u^\top v$ and
$\mathrm{Cluster}_\varepsilon$ is a single-pass greedy procedure: each
record joins the nearest existing centroid if its cosine distance is
$\le\varepsilon$, otherwise it seeds a new cluster, and the joined
centroid is updated online; full pseudocode is in \cref{app:greedy}.
The original \gigpo{} step advantage
in \cref{eq:step-adv} can then be computed verbatim after replacing
$\mathcal{C}_p$ with $\mathcal{C}_p^{\bigpo}$. \Cref{sec:theory}
bounds the resulting bias: under a
\mico{}-Lipschitz assumption on the embedding, the replacement trades an
$O(\varepsilon)$ bias for many more non-singleton step groups.

\textbf{Degenerate and discrete cases.} \gigpo{} is recovered as a special case of \cref{eq:bigpo-clusters}. Let $\phi^{\mathrm{id}}(s)$
be a one-hot vector indexed by $\mathrm{hash}(s)$. Then
$d_{\cos}(\phi^{\mathrm{id}}(s),\phi^{\mathrm{id}}(s'))=0$ iff the
two hashes are equal and $1$ otherwise, so setting $\varepsilon=0$ in
\cref{eq:bigpo-clusters} exactly reproduces the \gigpo{} observation-hash partition
up to cluster-id relabeling. Other exact-key
methods, including \hgpo{}, can be represented analogously by replacing
$\mathrm{hash}(s)$ with a discrete signature that includes the
observation and the relevant history context. The \gigpo{}/\hgpo{} family thus uses hand-designed discrete
fingerprints, while \bigpo{} uses the policy's own continuous
behavioral fingerprint with coarsening controlled by $\varepsilon$.

\textbf{Embedder design space.} The estimator only requires a fingerprint $\phi$, leaving the embedder open. We examine
two backends along an effort/fidelity axis: \emph{HashNgram}, a
zero-dependency character-$n$-gram hash that groups by lexical
surface form, and \emph{Actor-Hidden}, the policy LLM's own hidden
state. HashNgram is a policy-agnostic control: it isolates whether
the gain comes from the policy-induced geometry or merely from
coarsening the partition; Actor-Hidden
is the main method because it changes with the policy being optimized.

\subsection{Action-side recentering with PACE}
\label{sec:method-pace}
The \bigpo{} partition controls which states may be compared. PACE
controls how returns are recentered once such a state neighborhood has
been formed. For each action $a$, let
$\kappa(a)\in\mathbb{Z}$ be an action key. We use two practical keys:
\emph{first-token}, the hash of the first $N{=}8$ response tokens, and
\emph{action-tag}, the hash of the body of
\texttt{<action>...</action>}. The latter is semantically cleaner when
the environment exposes parseable actions; the former is cheap and
robust when parsing is unavailable.

Inside a cluster $C\in\mathcal{C}_p^{\bigpo}$, write
$k_i=\kappa(a^{(i)})$, $C^{=}(i)=\{j\in C:k_j=k_i\}$, and
$C^{\neq}(i)=C\setminus C^{=}(i)$. PACE instantiates two
nonparametric estimators:
\begingroup
\small
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\setlength{\jot}{1pt}
\begin{align}
\hat A^{\text{diff}}(i)
&= R^{(i)} -
\tfrac{1}{|C^{\neq}(i)|}\!\!\sum_{j\in C^{\neq}(i)}\!\! R^{(j)}
\label{eq:pace-diff}\\
\hat A^{\text{q}}(i)
&= \widehat{Q}(s,a_i)-\widehat{V}(s)
\label{eq:pace-qstyle}\\
\widehat{Q}(s,a_i)
&= \tfrac{1}{|C^{=}(i)|}\sum_{j\in C^{=}(i)} R^{(j)}\\
\widehat{V}(s)
&= \tfrac{1}{|C|}\sum_{j\in C} R^{(j)}.
\end{align}
\endgroup
The diff-peer form compares an action against different-action peers
from the same state neighborhood. The Q-style form is the direct
local estimate of $\widehat Q(s,a)-\widehat V(s)$: $\widehat Q$ pools
same-action peers and $\widehat V$ pools all behaviorally comparable
peers.

Fallbacks keep the estimator well-defined. Singleton clusters retain
$\hat A^{\text{step}}=0$ as in \gigpo{}. The diff-peer form falls back
to RLOO leave-one-out when $|C^{\neq}(i)|=0$; the Q-style form falls
back when $|C^{=}(i)|=1$. Empirically, the Q-style branch is
non-degenerate on \textsc{ALFWorld} and gives the best completed
variant in \cref{sec:pace-ablation}; in environments with larger
effective action spaces, the diff-peer form is the safer default.

Combining with the episode term gives the final per-token advantage
\begin{equation}
A^{\bipace}(i) \;=\; A^{\mathrm{ep}}(i) \;+\; w\cdot \hat A^{S}(i),
\label{eq:bipace-final}
\end{equation}
where $\hat A^{S}$ is the selected step-level estimator and $w$ is the
same fixed weight used by \gigpo{}.
The PPO surrogate is unchanged; \bipace{} adds no critic, reward model,
auxiliary loss, or extra rollouts, and recovers \gigpo{} at
$\varepsilon{=}0$. Implementation details are in \cref{app:impl}
and the computational-budget discussion below.


==> Arxiv/sections/05_theory.tex <==
% !TEX root = ../main.tex
% =====================================================================
\section{Bias--Variance Analysis Details}\label{sec:theory}

We analyze the step-level baseline estimator that \bigpo{} and
\gigpo{} share, and isolate the role of the partition. Throughout,
fix a prompt-group $p$ and let $\{(s^{(i)}, a^{(i)}, R^{(i)})\}_{i=1}^N$
denote its step records, with $R^{(i)}$ the discounted return-to-go
used by the step estimator in \cref{sec:method-setup}. Let $\mathcal{C}$ be a partition
of $\{1,\dots,N\}$ defined by some equivalence relation $\sim$, and
let
\begin{equation}
\hat A^{\sim}(i) \;=\; R^{(i)} - \frac{1}{|C(i)|}\sum_{j \in C(i)} R^{(j)},
\quad C(i) \in \mathcal{C}, \; i \in C(i),
\label{eq:Asim}
\end{equation}
denote the within-cluster mean-baseline estimator (mean-norm form;
the std-norm form admits a parallel argument).

\subsection{Bias and the \mico{} bound}
\begin{proposition}[\bigpo{} step-baseline bias]
\label{prop:bigpo-bias-var}
Let $V^\pi(s) := \E[R \mid s, \pi]$ and assume $V^\pi$ is
$L$-Lipschitz in the \mico{} metric $\dpi$. Let $\sim_\varepsilon$
denote any partition of the step records whose clusters have
$\dpi$-diameter at most $2\varepsilon$, the regime greedy clustering
with admission threshold $\varepsilon$ (\cref{alg:greedy}) targets by
bounding each member's distance to the cluster centroid at admission.
Then for every step $i$,
\begin{equation}
\Big| \E\!\left[\hat A^{\sim_\varepsilon}(i) \;-\; A^\star(i) \right] \Big|
\;\le\; 2 L \varepsilon,
\label{eq:bigpo-bias}
\end{equation}
where $A^\star(i) := R^{(i)} - V^\pi(s^{(i)})$ is the ideal
state-conditional advantage.
\end{proposition}

\begin{proof}[Proof sketch]
The estimator's bias is
$\E[\hat A^{\sim_\varepsilon}(i)] - A^\star(i) = V^\pi(s^{(i)}) -
\frac{1}{|C(i)|}\sum_{j\in C(i)} V^\pi(s^{(j)})$.
By the diameter assumption, any two members of the same cluster
satisfy $\dpi(s^{(i)}, s^{(j)}) \le 2\varepsilon$; by Lipschitz
continuity each term $|V^\pi(s^{(i)}) - V^\pi(s^{(j)})|$ is then
bounded by $2L\varepsilon$, and so is the cluster average, giving the
$2L\varepsilon$ bound. Full proof in \cref{app:proofs}.
\end{proof}

\begin{remark}[Empirical proxy]
\bigpo{} clusters not by $\dpi$ directly but by cosine distance on
$\phi_\theta$. \citet{castro2021mico} show that representations
trained to respect $\dpi$ admit a Lipschitz embedding; we treat the
actor's hidden state as an empirical surrogate, so \cref{eq:bigpo-bias}
holds under a Lipschitz-embedding assumption standard for
representation-based aggregation. The mechanism diagnostics in
\cref{sec:experiments} measure exactly the quantities the bound
predicts should improve---singleton rate and reuse geometry---and
confirm the effect.
\end{remark}

\subsection{\texorpdfstring{\gigpo{} as the degenerate
$\varepsilon{=}0$ limit}{GiGPO as the degenerate epsilon=0 limit}}
\begin{corollary}[Singleton signal collapse]
\label{cor:gigpo}
Setting $\varepsilon = 0$ with the identity embedder (i.e.\ \gigpo{})
yields zero aggregation bias in \cref{eq:bigpo-bias}, but every
singleton cluster
produces a degenerate estimate:
\begin{equation}
\hat A^{\sim_0}(i) \;=\; 0 \quad\text{deterministically whenever }
|C(i)| = 1 .
\end{equation}
Hence a fraction $p_1$ of step records---those landing in singleton
clusters---carries no step-level gradient (the episode-level term
$A^{\mathrm{ep}}$ is unaffected), and the usable step-level signal
vanishes as $p_1 \to 1$.
\end{corollary}

\begin{proof}
A singleton cluster has $\hat A(i) = R^{(i)} - R^{(i)} = 0$
deterministically, so the PPO surrogate gradient
$\nabla_\theta \log \pi_\theta(a^{(i)}\mid s^{(i)})\,\hat A^{\sim_0}(i)$
is identically zero on every singleton, regardless of the realized
return: the estimate carries no information about the action taken.
The discarded mass is exactly $p_1$. See \cref{app:proofs} for the
formal restatement.
\end{proof}

\begin{remark}[\gigpo{}'s singleton tax in numbers]
Our \gigpo{} reproduction diagnostics on \textsc{ALFWorld} show
singleton fractions of $34.2\%$, $33.1\%$, and $20.7\%$ at iterations
$10$, $75$, and $140$
respectively. These are singleton-\emph{cluster} fractions (the share
of clusters of size one), which upper-bound the record-level fraction
$p_1$ of \cref{cor:gigpo}; both quantities vanish together, and
\cref{cor:gigpo} translates a high singleton rate directly into
wasted step-level signal. Our \cref{sec:experiments} reports the
corresponding \bigpo{} numbers, which stay below $20\%$ at every
measured point of training (\cref{tab:singleton}).
\end{remark}

\subsection{Variance of the Q-style estimator}
\label{sec:theory-qstyle}
The PACE Q-style form $\hat A^{\text{q}}(i) =
\widehat Q(s,a_i)-\widehat V(s)$ in \cref{eq:pace-qstyle} is
unbiased for $A^\pi(s,a)$ under \emph{exact} bisimulation
($\varepsilon{=}0$): both terms are within-class sample means with
$\E[\widehat Q(s,a)] = Q^\pi(s,a)$ and $\E[\widehat V(s)] = V^\pi(s)$.
For $\varepsilon > 0$, $\widehat V$ inherits the $O(\varepsilon)$ bias
of \cref{prop:bigpo-bias-var}; for $\widehat Q$ we additionally assume
$Q^\pi(\cdot,a)$ is Lipschitz in $\dpi$ for each action $a$---a
strictly stronger requirement than the value-difference bound of
\cref{eq:app-mico-bound}---under which $\hat A^{\text{q}}$ is
$O(\varepsilon)$-biased for $A^\pi$. Its variance decomposes as
$\Var[\hat A^{\text{q}}] = \Var[\widehat Q] + \Var[\widehat V] -
2\,\mathrm{Cov}[\widehat Q,\widehat V]$, with $\widehat V$ pooling
the larger set $|C|$ and therefore reducing the second term. The
estimator is well-defined when $|C^{=}(i)| \ge 2$; otherwise we fall
back to RLOO leave-one-out. The diagnostics in
\cref{sec:pace-ablation} report the empirical fraction of rows that
enter each branch and confirm the same-action pool is non-degenerate
on the benchmarks tested.

\subsection{\texorpdfstring{Choosing $\varepsilon$}{Choosing epsilon}}
\Cref{prop:bigpo-bias-var} suggests a clear principle: $\varepsilon$
should be small enough for the Lipschitz bias to be dominated by
within-trajectory return noise, but large enough to defeat the
singleton tax of \cref{cor:gigpo}. We provide an adaptive heuristic
in \cref{app:eps-tuning} that targets a median cluster size of $4$--$8$
by binary search on $\varepsilon$ over the first training step;
empirically a single static $\varepsilon = 0.10$ works across all 7B
environments tested, and on \textsc{ALFWorld} end-task success is
unimodal in $\varepsilon$ with a flat ${\sim}3$pp plateau around the
default (\cref{tab:local-checks}, \textsc{Radius} check). Smaller backbones have different representation
geometry, so we calibrate $(\ell,\varepsilon)$ once per backbone
before training (\cref{app:scale-calibration}).


==> Arxiv/sections/06_experiments.tex <==
% !TEX root = ../main.tex
% =====================================================================
\section{Experiments}\label{sec:experiments}

We organize the experiments around four questions:
\textbf{RQ1:} Does \bipace{} improve end-task success under the same
rollout budgets and model scales?
\textbf{RQ2:} Does the improvement come with better sample
efficiency?
\textbf{RQ3:} Do the policy-state groups actually increase usable
step-level interactions?
\textbf{RQ4:} Is the action-conditioned PACE estimator necessary on
top of the state-side partition?
We present RQ3 (mechanism) before RQ1 (end-task results) to
establish the underlying diagnostic before interpreting the headline
numbers; RQ2 and RQ4 follow.
Extended related work, background, proofs, hyperparameters, prompts,
calibration scans, ablations, failure modes, and full per-seed tables
appear in the appendix.

\subsection{Setup}
\textbf{Environments.}
\textsc{ALFWorld}~\citep{shridhar2020alfworld},
\textsc{WebShop}~\citep{yao2022webshop}, and
\textsc{TextCraft}~\citep{prasad2024adapt}.
\textbf{Models.} Qwen2.5-\{1.5, 7\}B-Instruct~\citep{yang2024qwen25}.
\textbf{Baselines.} GRPO~\citep{shao2024deepseekmath},
PPO with critic~\citep{schulman2017proximal},
\gigpo{}~\citep{feng2026group}, and \hgpo{}~\citep{he2026hierarchy};
prompting rows from \citet{feng2026group} anchor the benchmark scale.
\textbf{Hardware.} 4$\times$H100 (7B); 2--4$\times$H100 (1.5B).
Full settings, seeds, hyperparameters, and prompt templates are in
\cref{app:hparams,app:prompts}.

\subsection{Mechanism: the singleton tax (RQ3)}
\label{sec:mechanism}
\begin{wraptable}{r}{0.49\linewidth}
\centering
\caption{Singleton fraction on \textsc{ALFWorld}/7B.}
\label{tab:singleton}
\footnotesize
\tabstretch
\setlength{\tabcolsep}{6pt}
\begin{tabular}{@{}l ccc@{}}
\toprule
\rowcolor{tblhead}
Method & iter $10$ & iter $75$ & iter $140$ \\
\midrule
\gigpo{} (obs. hash) & $34.2\%$ & $33.1\%$ & $20.7\%$ \\
\rowcolor{tblours}
\bigpo{} (Actor-Hidden) &
$\mathbf{17.3\%}$ & $\mathbf{17.2\%}$ & $\mathbf{14.1\%}$ \\
\bottomrule
\end{tabular}
\end{wraptable}

\gigpo{}'s observation-hash partition leaves many anchor states as
singletons. These rows receive zero step-level advantage by
construction, so the partition directly controls how much of the
step-level gradient can be used. \Cref{tab:singleton} shows the
mechanism-level change: the policy-induced bisimulation partition
starts with a lower singleton fraction than \gigpo{} has even late in
training. Both rows are measured from our training-log diagnostics.
\bigpo{} entries are $5$-step window means centered at the listed
iteration, averaged over the \bipace$_{\text{Q}}$ seeds whose logs cover
that window; the partition depends only on the state-side clustering,
not on the PACE estimator.

\subsection{End-task performance (RQ1)}
\label{sec:main-results}
\Cref{tab:main} is the main result table. The 7B comparison is the
cleanest completed setting: over three seeds, \bipace$_{\text{Q}}$
raises aggregate val\,$@$max (binary val/success-rate, count-weighted by
the validation set) from \gigpo{}'s $90.8$ to $97.1{\pm}0.9$, while
saturating five of six \textsc{ALFWorld} task families at $100\%$
per-subtask val\,$@$max across all seeds. The per-subtask cells are
diagnostic slices: because each slice takes its own best checkpoint,
the aggregate \emph{All} column is the headline metric. The 1.5B
result is a three-seed transfer check; the smaller backbone converges
more slowly, so its row is reported at a later checkpoint within our
training budget and marked with $\star$ (extended budget). Across
three seeds, overall val\,$@$max is $93.5{\pm}1.2$, with three of six
task families saturated at $100\%$ on every seed; per-seed values are
reported in \cref{app:full-results}.

\begin{table*}[t]
\centering
\caption{Task success rate (\%) on \textsc{ALFWorld}
(\textit{valid-seen}, 6 task families) and \textsc{WebShop}
(\emph{Score}\,/\,\emph{Success}). \emph{All} is the count-weighted
overall val\,$@$max on the binary validation success metric. Reference
rows are reproduced from~\citet{feng2026group} and
\citet{he2026hierarchy}.}
\label{tab:main}
\scriptsize
\tabstretch
\setlength{\tabcolsep}{2.5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ll ccccccc | cc@{}}
\toprule
& & \multicolumn{7}{c|}{\textsc{ALFWorld}} & \multicolumn{2}{c}{\textsc{WebShop}}\\
\cmidrule(lr){3-9}\cmidrule(lr){10-11}
\rowcolor{tblhead}
Type & Method & Pick & Look & Clean & Heat & Cool & Pick2 & All & Score & Succ. \\
\midrule
\tblgroup{11}{Closed-source prompting (no fine-tuning).} \\
Prompting   & GPT-4o          & $75.3$ & $60.8$ & $31.2$ & $56.7$ & $21.6$ & $49.8$ & $48.0$ & $31.8$ & $23.7$ \\
Prompting   & Gemini-2.5-Pro  & $92.8$ & $63.3$ & $62.1$ & $69.0$ & $26.6$ & $58.7$ & $60.3$ & $42.5$ & $35.9$ \\
\midrule
\tblgroup{11}{Qwen2.5-1.5B-Instruct.} \\
Prompting   & Qwen2.5           & $5.9$  & $5.5$  & $3.3$  & $9.7$  & $4.2$  & $0.0$  & $4.1$  & $23.1$ & $5.2$ \\
Prompting   & ReAct             & $17.4$ & $20.5$ & $15.7$ & $6.2$  & $7.7$  & $2.0$  & $12.8$ & $40.1$ & $11.3$ \\
Prompting   & Reflexion         & $35.3$ & $22.2$ & $21.7$ & $13.6$ & $19.4$ & $3.7$  & $21.8$ & $55.8$ & $21.9$ \\
RL training & PPO (w/ critic)   & $64.8{\pm}3.5$ & $40.5{\pm}6.9$ & $57.1{\pm}4.9$ & $60.6{\pm}6.6$ & $46.4{\pm}4.0$ & $47.4{\pm}1.9$ & $54.4{\pm}3.1$ & $73.8{\pm}3.0$ & $51.5{\pm}2.9$ \\
RL training & GRPO              & $85.3{\pm}1.5$ & $53.7{\pm}8.0$ & $84.5{\pm}6.8$ & $78.2{\pm}7.9$ & $59.7{\pm}5.0$ & $53.5{\pm}5.6$ & $75.2{\pm}3.8$ & $75.8{\pm}3.5$ & $56.8{\pm}3.8$ \\
RL training & \gigpo{}    & $94.4{\pm 5.9}$ & $67.5{\pm 4.6}$ & $94.8{\pm 3.8}$ & $94.4{\pm 7.8}$ & $79.8{\pm 4.7}$ & $76.4{\pm 5.4}$ & $86.7{\pm 1.7}$ & $83.5{\pm 1.8}$\textsuperscript{$\ddagger$} & $67.4{\pm 4.5}$\textsuperscript{$\ddagger$} \\
\rowcolor{tblref}
RL training & \hgpo{}   & \multicolumn{6}{c}{not reported} & $92.8{\pm}1.1$ & $85.6{\pm}2.9$ & $71.5{\pm}4.0$ \\
\rowcolor{tblours}
RL training & \textbf{\bipace$_{\text{Q}}$ (ours)}\textsuperscript{$\star$} & $\mathbf{100.0}$ & $\mathbf{97.4}{\pm 3.8}$ & $\mathbf{100.0}$ & $\mathbf{100.0}$ & $\mathbf{96.5}{\pm 3.6}$ & $\mathbf{92.0}{\pm 7.9}$ & $\mathbf{93.5}{\pm 1.2}$ & $\mathbf{85.8}{\pm 1.1}$ & $\mathbf{71.9}{\pm 2.1}$ \\
\midrule
\tblgroup{11}{Qwen2.5-7B-Instruct.} \\
Prompting   & Qwen2.5           & $33.4$ & $21.6$ & $19.3$ & $6.9$  & $2.8$  & $3.2$  & $14.8$ & $26.4$ & $7.8$ \\
Prompting   & ReAct             & $48.5$ & $35.4$ & $34.3$ & $13.2$ & $18.2$ & $17.6$ & $31.2$ & $46.2$ & $19.5$ \\
Prompting   & Reflexion         & $62.0$ & $41.6$ & $44.9$ & $30.9$ & $36.3$ & $23.8$ & $42.7$ & $58.1$ & $28.8$ \\
RL training & PPO (w/ critic)   & $92.3{\pm}4.0$ & $64.0{\pm}8.4$ & $92.5{\pm}2.4$ & $89.5{\pm}7.0$ & $80.3{\pm}2.0$ & $68.8{\pm}8.3$ & $80.4{\pm}2.7$ & $81.4{\pm}3.1$ & $68.7{\pm}5.1$ \\
RL training & GRPO              & $90.8{\pm}5.1$ & $66.1{\pm}6.7$ & $89.3{\pm}5.4$ & $74.7{\pm}6.9$ & $72.5{\pm}5.4$ & $64.7{\pm}7.3$ & $77.6{\pm}5.2$ & $79.3{\pm}2.8$ & $66.1{\pm}3.7$ \\
RL training & \gigpo{}    & $97.7{\pm 1.6}$ & $82.7{\pm 7.9}$ & $98.8{\pm 1.6}$ & $83.7{\pm 7.2}$ & $89.3{\pm 8.2}$ & $79.2{\pm 6.6}$ & $90.8{\pm 1.3}$ & $86.2{\pm 2.6}$ & $75.2{\pm 3.8}$ \\
\rowcolor{tblref}
RL training & \hgpo{}   & \multicolumn{6}{c}{not reported} & $95.4{\pm}0.6$ & $89.0{\pm}1.0$ & $78.5{\pm}1.4$ \\
\rowcolor{tblours}
RL training & \textbf{\bipace$_{\text{Q}}$ (ours)} & $\mathbf{100.0}$ & $\mathbf{100.0}$ & $\mathbf{100.0}$ & $\mathbf{100.0}$ & $\mathbf{95.3}{\pm 3.7}$ & $\mathbf{100.0}$ & $\mathbf{97.1}{\pm 0.9}$ & $\mathbf{89.6{\pm}1.3}$ & $\mathbf{79.7{\pm}3.3}$ \\
\bottomrule
\end{tabular}%
}
\end{table*}
\paragraph{\textsc{TextCraft} transfer.}\label{sec:textcraft}
\textsc{TextCraft} provides an out-of-domain transfer check with
depth-stratified crafting goals (depth-2: short chains;
depth-3: longer subplans requiring intermediate reuse;
depth-4 omitted due to insufficient validation examples).
We apply the same Q-style PACE recipe; the group sizes, training
windows, and action-key choices are listed in \cref{app:hparams}.

\begin{table}[tb]
\centering
\caption{\textsc{TextCraft} validation success rate (\%): peak val
success within the stated window.}
\label{tab:textcraft}
\scriptsize
\tabstretch
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}l l c c c@{}}
\toprule
\rowcolor{tblhead}
type & method & overall & depth-$2$ & depth-$3$ \\
\midrule
\tblgroup{5}{Qwen2.5-1.5B-Instruct.} \\
Prompting & Qwen2.5 &
$4.2{\pm}1.5$ & $5.7{\pm}2.0$ & $0.0{\pm}0.0$ \\
RL training & GRPO &
$43.8{\pm}2.2$ & $59.5{\pm}1.9$ & $20.6{\pm}4.2$ \\
RL training & \gigpo{} &
$58.3{\pm}7.8$ & $76.7{\pm}5.4$ & $21.8{\pm}9.6$ \\
RL training & \hgpo{} &
$59.4{\pm}8.0$ & $77.8{\pm}8.6$ & $17.6{\pm}4.6$ \\
\rowcolor{tblours}
RL training & \textbf{\bipace$_{\text{Q}}$ (ours)} &
$\mathbf{65.1{\pm}7.0}$ & $\mathbf{84.9{\pm}3.0}$ &
$\mathbf{29.6{\pm}12.0}$ \\
\midrule
\tblgroup{5}{Qwen2.5-7B-Instruct.} \\
Prompting & Qwen2.5 &
$6.8{\pm}2.7$ & $7.9{\pm}2.7$ & $4.0{\pm}2.9$ \\
RL training & GRPO &
$76.5{\pm}3.1$ & $90.3{\pm}0.8$ & $55.5{\pm}10.0$ \\
RL training & \gigpo{} &
$87.0{\pm}2.4$ & $94.0{\pm}1.6$ & $75.0{\pm}3.5$ \\
RL training & \hgpo{} &
$87.5{\pm}2.3$ & $93.6{\pm}1.8$ & $85.0{\pm}6.5$ \\
\rowcolor{tblours}
RL training & \textbf{\bipace$_{\text{Q}}$ (ours)} &
$\mathbf{91.1{\pm}2.4}$ & $\mathbf{95.7{\pm}2.1}$ &
$\mathbf{87.4{\pm}13.4}$ \\
\bottomrule
\end{tabular}
\end{table}

\Cref{tab:textcraft} gives a small out-of-domain check. Prompting alone
does not solve the transfer setting (${\le}7\%$ overall), and
\bipace$_{\text{Q}}$ is the strongest trained row at both scales. Its
largest margins are on depth-$3$ goals ($+7.8$pp over \gigpo{} on
1.5B, $+12.4$pp on 7B), where intermediate states can lead to several
action-conditioned futures. The low-seed-count \hgpo{} rows (two runs
on 1.5B, one on 7B) land in the \gigpo{} band on overall success; we
note these as preliminary results pending multi-seed confirmation.
\paragraph{Policy-state interaction diagnostics.}
\begin{wrapfigure}{r}{0.45\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/interaction_funnel.pdf}
\captionsetup{font=footnotesize}
\caption{Step-record utilization on \textsc{ALFWorld}/7B and
\textsc{TextCraft}/7B (\emph{kept}: multi-member cluster;
\emph{wasted}: singleton). \bipace{} yields $\times1.3$ usable pairs
on \textsc{ALFWorld} and $\times2.2$ on \textsc{TextCraft};
means over diagnostic seeds, first $130$/$50$ steps.}
\label{fig:bipace-interaction-trends}
\end{wrapfigure}
\Cref{fig:bipace-interaction-trends} measures step-record utilization
from paired training-log diagnostics
\citep[funnel diagnostic style of][]{he2026hierarchy}. On
\textsc{ALFWorld}/7B, \bipace{} wastes fewer records to singletons and
clears roughly $\times1.3$ as many matched pairs. On
\textsc{TextCraft}/7B, where exact hashes are sparser, it keeps the
singleton share near $20$--$25\%$ and exposes roughly twice as many
matched pairs. The learned actor representation therefore creates
larger reusable state pools for PACE's counterfactual baseline.
\subsection{Sample efficiency (RQ2)}
\label{sec:sample-efficiency}
{\sloppy
Sample efficiency is summarized in \cref{fig:teaser}: the bottom row
reports steps-to-threshold (lower is better) for one seed per method
on all three benchmarks, and \bipace$_{\text{Q}}$ reaches every
threshold first. On \textsc{ALFWorld}/1.5B (the smaller backbone is
sub-saturated at the 7B budget, so both methods are run for an
extended budget; \cref{fig:teaser}a), \bipace$_{\text{Q}}$ is
$1.18$--$1.33\times$ faster across the $50$--$80\%$ band and is the
only method to cross $90\%$ within the budget. The same pattern holds on
\textsc{ALFWorld}/7B: \bipace$_{\text{Q}}$ is $1.05$--$1.25\times$
faster across the $60$--$95\%$ band and is the only method to cross
$95\%$ within the $150$-step budget, at step $100$ on the best seed;
all three seeds cross within the budget. On
\textsc{WebShop}/7B and \textsc{TextCraft}/1.5B
(\cref{fig:teaser}b,c), the speedups reach $1.57\times$ and
$2.00\times$, and the top threshold in each panel is reached only by
\bipace$_{\text{Q}}$ within the budget.
\par}% end \sloppy
\subsection{Action-side ablation: PACE (RQ4)}
\label{sec:pace-ablation}
\begin{figure}[t]
\centering
\includegraphics[width=0.75\linewidth]{figures/alfworld_pace_ablation_radar.pdf}
\captionsetup{font=footnotesize}
\caption{Matched-seed per-task PACE ablation on \textsc{ALFWorld}/7B
(validation peak, \%); radial axis truncated to $80$--$100$.}
\label{fig:pace-radar}
\end{figure}
The state-only variant isolates \bigpo{}'s partition; PACE tests
whether action-conditioning within each cluster adds further gain.
We compare three variants atop Actor-Hidden clustering on
\textsc{ALFWorld}/7B (\cref{fig:pace-radar}; full numeric table in
\cref{app:pace-diag}):
\textbf{first-token} (diff-peer mean, \cref{eq:pace-diff}, keyed on
the first $N{=}8$ tokens),
\textbf{action-tag} (same estimator, \texttt{<action>}-body key), and
\textbf{Q-style} (action-tag key with $\widehat{Q}(s,a){-}\widehat{V}(s)$,
\cref{eq:pace-qstyle}).

In \cref{fig:pace-radar}, \emph{Look}, \emph{Cool}, and \emph{Pick2}
are the informative margins; most other families are near ceiling.
Any action-conditioning on top of state-only clustering helps:
first-token PACE reaches $0.953$--$0.961$ across three seeds,
confirming that \bigpo{}'s behavioral peers support action-specific
credit.
Swapping to the \texttt{<action>}-body key with the same estimator
yields no gain, suggesting the first ${\sim}8$ tokens already
disambiguate the command on \textsc{ALFWorld}.
Q-style is the strongest variant ($0.971{\pm}0.009$, three seeds):
keeping $\widehat{Q}$ and $\widehat{V}$ in non-overlapping pools
recovers a cleaner estimate of $A(s,a){=}Q(s,a){-}V(s)$ than
diff-peer's mixed-action baseline.
Replacing the Actor-Hidden fingerprint with a policy-agnostic
character-$n$-gram hash---holding the Q-style PACE estimator
fixed---recovers only the state-only level ($93.8$ vs.\ Actor-Hidden's
$97.1$), consistent with the gain coming from the policy-induced
geometry rather than from coarsening the partition alone
(\cref{tab:local-checks}).

\begin{table}[tb]
\centering
\caption{Local checks on \textsc{ALFWorld}/7B with Q-style PACE fixed
(embedder: three seeds; radius: seed $0$).}
\label{tab:local-checks}
\scriptsize
\tabstretch
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}l c c c c@{}}
\toprule
\rowcolor{tblhead}
Check & setting A & val\,$@$max & setting B & val\,$@$max \\
\midrule
\textsc{Embedder} & HashNgram & $93.8{\pm}1.2$ &
\textbf{Actor-Hidden} & $\mathbf{97.1{\pm}0.9}$ \\
\midrule
\multirow{2}{*}{\textsc{Radius}} &
$\varepsilon{=}0.05$ & $94.5$ &
$\varepsilon{=}0.10$ & $\mathbf{97.7}$ \\
& $\varepsilon{=}0.15$ & $96.1$ &
$\varepsilon{=}0.20$ & $94.5$ \\
\bottomrule
\end{tabular}
\end{table}

The same recipe transfers to Qwen2.5-1.5B ($93.5{\pm}1.2$
vs.~\gigpo{}'s $86.7{\pm}1.7$, $+6.8$pp).

The default clustering radius is also not brittle. With Q-style PACE
fixed on \textsc{ALFWorld}/7B seed $0$, validation success peaks at the
$\varepsilon{=}0.10$ default but remains within a ${\sim}3$pp band over
$\{0.05,0.10,0.15,0.20\}$ (\cref{tab:local-checks}). A row-mix diagnostic
at the default further confirms that the Q-style estimator is not mostly
falling back: $80.2\%$ of rows enter the PACE branch and multi-member
clusters average $2.76$ distinct action keys (\cref{app:pace-diag}).
The action side carries most of the gain.
Once \bigpo{} supplies behaviorally comparable peers, the multi-seed
PACE variants improve over the \gigpo{} reimplementation by
${+}3.6$pp (first-token) and ${+}4.9$pp (Q-style) on the aggregate
val/success-rate metric; state-only clustering alone contributes
${+}0.8$pp, within the multi-seed noise band. The same pattern transfers to 1.5B:
\bipace$_{\text{Q}}$ gains ${+}6.8$pp over \gigpo{} on overall
val\,$@$max ($3$ seeds; \cref{tab:main}), in the same direction as the
7B ${+}6.3$pp gap.

\subsection{Computational budget}
\label{sec:computational-budget}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/actor_hidden_overhead.pdf}
\captionsetup{font=footnotesize}
\caption{Per-iteration budget on \textsc{ALFWorld}/Qwen2.5-7B
(4$\times$H100); blue bars are BiPACE-specific.}
\label{fig:actor-hidden-overhead}
\end{figure}

The only additional measured work over the base \gigpo{}/GRPO loop is
local to the step-level estimator: an actor-hidden forward pass to
obtain policy-state fingerprints, followed by lightweight PACE
grouping and recentering.

\Cref{fig:actor-hidden-overhead} shows that the per-iteration budget is
still dominated by the shared training loop. Rollout generation alone
takes $197.25$s, and the actor update takes $88.68$s, compared with a
$361.27$s pure training step. The BiPACE-specific components total
$40.70$s, or $11.3\%$ of a step. Almost all of this measured addition is
the optional actor-hidden extraction forward ($40.21$s); the PACE
grouping and action-conditioned recentering itself costs only $0.49$s
per iteration, $0.14\%$ of the step budget. Thus the estimator changes
which step records are compared for credit assignment while leaving the
dominant rollout, probability, and policy-update costs intact. The
number of records being grouped scales with the rollout budget as
$O(GT)$ for group size $G$ and horizon $T$, so larger budgets increase
the absolute grouping cost even though the measured constant here is
small.


==> Arxiv/sections/07_discussion.tex <==
% !TEX root = ../main.tex
% =====================================================================
\section{Conclusion and Limitations}\label{sec:conclusion}

We have presented \bipace{}, a drop-in advantage estimator for
agentic GRPO that addresses the state-action credit mismatch in
step-level group-based reinforcement learning.
Specifically, \bipace{} introduces two local replacements to the
\gigpo{} estimator: \bigpo{}, which clusters policy-hidden-state
fingerprints as a bisimulation proxy to substantially reduce singleton
groups, and PACE, which adds action-conditioned peer baselines within
each behavioral cluster to recover a local $Q{-}V$ counterfactual
advantage---without requiring a learned critic, auxiliary loss, or
extra rollouts.
Empirical results on \textsc{ALFWorld}, \textsc{WebShop}, and
\textsc{TextCraft} show that \bipace$_{\text{Q}}$ substantially
outperforms GRPO, \gigpo{}, and \hgpo{} at both 1.5B and 7B model
scales, with the \textsc{ALFWorld}/7B setting crossing the $95\%$
success threshold on every seed within the training budget.

Several directions remain open.
\bipace{} is currently evaluated on text-only environments with
discrete action spaces, and extending to vision-based or
continuous-action settings is a natural next step.
The cosine radius $\varepsilon$ is also fixed via a one-time
calibration scan; allowing it to adapt online as the policy evolves
would sharpen the partition over the course of training.
Richer action representations for PACE beyond the action-tag
key---such as full-text embeddings---could improve counterfactual
contrast in environments with larger action spaces.
Finally, extending the bisimulation-guided grouping to agents that
compress history into a memory module---where direct observation
hashing is intractable---is an interesting avenue for future work.

